sl(N)-Web categories

In this paper we use colored sl(N)-matrix factorizations, due to Wu and Y.Y., in order to categorify part of the quantum skew Howe duality defined by Cautis, Kamnitzer and Morrison. In particular, we define web categories and 2-representations of Khovanov and Lauda's categorical quantum sl(m) on them. We show that each such web category is equivalent to the category of finite dimensional graded projective modules over a certain level N cyclotomic Khovanov-Lauda-Rouquier algebra.

==> figure/e-i.tex <==
\unitlength 0.1in
\begin{picture}(6.00,3.00)(1.500,-6.500)
\special{pn 8}%
\special{pa 400 800}%
\special{pa 400 400}%
\special{fp}%
\special{sh 1}%
\special{pa 400 400}%
\special{pa 380 468}%
\special{pa 400 454}%
\special{pa 420 468}%
\special{pa 400 400}%
\special{fp}%
\put(4.0000,-8.50000){\makebox(0,0){${}_{i}$}}%
\put(5.0000,-6.0000){\makebox(0,0){${}_{{\lambda}}$}}%
\end{picture}%


==> figure/f-i.tex <==
\unitlength 0.1in%
\begin{picture}(6.00,3.00)(1.500,-6.500)
\put(4.0000,-8.50000){\makebox(0,0){${}_{i}$}}%
\put(5.0000,-6.0000){\makebox(0,0){${}_{{\lambda}}$}}%
\special{pn 8}%
\special{pa 400 390}%
\special{pa 400 800}%
\special{fp}%
\special{sh 1}%
\special{pa 400 800}%
\special{pa 420 734}%
\special{pa 400 748}%
\special{pa 380 734}%
\special{pa 400 800}%
\special{fp}%
\end{picture}%


==> figure/line-cross1.tex <==
\unitlength 0.1in
\begin{picture}(  6.0000,  4.0000)(  1.0000, -6.0000)
\special{pn 8}%
\special{pa 400 600}%
\special{pa 400 200}%
\special{fp}%
\special{pn 8}%
\special{pa 200 600}%
\special{pa 400 300}%
\special{dt 0.045}%
\put(4.0000,-1.0000){\makebox(0,0){${}_{a}$}}%
\put(2.0000,-5.0000){\makebox(0,0){${}_{N}$}}%
\put(4.0000,-7.0000){\makebox(0,0){${}_{N-a}$}}%
\end{picture}%


==> figure/line-cross3.tex <==
\unitlength 0.1in
\begin{picture}(  6.0000,  4.0000)(  1.0000, -6.0000)
\special{pn 8}%
\special{pa 400 600}%
\special{pa 400 200}%
\special{fp}%
\special{pn 8}%
\special{pa 600 600}%
\special{pa 400 300}%
\special{dt 0.045}%
\put(4.0000,-1.0000){\makebox(0,0){${}_{a}$}}%
\put(6.0000,-5.0000){\makebox(0,0){${}_{N}$}}%
\put(4.0000,-7.0000){\makebox(0,0){${}_{N-a}$}}%
\end{picture}%


==> figure/line.tex <==
\unitlength 0.1in
\begin{picture}(  2.0000,  4.0000)(  1.0000, -6.0000)
\special{pn 8}%
\special{pa 200 600}%
\special{pa 200 200}%
\special{fp}%
\special{sh 1}%
\special{pa 200 200}%
\special{pa 180 268}%
\special{pa 200 254}%
\special{pa 220 268}%
\special{pa 200 200}%
\special{fp}%
\put(2.0000,-1.0000){\makebox(0,0){${}_{a}$}}%
\end{picture}%

